GarNet: A Two-Stream Network for Fast and Accurate 3D Cloth Draping

While Physics-Based Simulation (PBS) can accurately drape a 3D garment on a 3D body, it remains too costly for real-time applications, such as virtual try-on. By contrast, inference in a deep network, requiring a single forward pass, is much faster. Taking advantage of this, we propose a novel architecture to fit a 3D garment template to a 3D body. Specifically, we build upon the recent progress in 3D point cloud processing with deep networks to extract garment features at varying levels of detail, including point-wise, patch-wise and global features. We fuse these features with those extracted in parallel from the 3D body, so as to model the cloth-body interactions. The resulting two-stream architecture, which we call as GarNet, is trained using a loss function inspired by physics-based modeling, and delivers visually plausible garment shapes whose 3D points are, on average, less than 1 cm away from those of a PBS method, while running 100 times faster. Moreover, the proposed method can model various garment types with different cutting patterns when parameters of those patterns are given as input to the network.

==> fig/curvesAblationUCL.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}[htbp]
	\centering
	\begin{tabular}{cc}
		\includegraphics[width=0.23\textwidth]{visuals/ablationUCL/distCurveUCL.pdf}&
		\includegraphics[width=0.23\textwidth]{visuals/ablationUCL/angleCurveUCL.pdf}\\
	\end{tabular}
	
	\caption{\small \textbf{Ablation study for the loss terms}: Average precision curves for the vertex distance and the facet normal angle error. The distance is unitless since the actual measurements are not reported by~\cite{Wang18}. Best viewed in color.}
	\label{fig:ablationUCL}
\end{figure}

%\begin{figure*}[htbp]
%	\centering
%	\begin{tabular}{cccc}
%		\includegraphics[width=0.24\textwidth]{visuals/FJWdistCurve.pdf}&
%		\includegraphics[width=0.24\textwidth]{visuals/FJWangleCurve.pdf}&
%		\includegraphics[width=0.24\textwidth]{visuals/MJWdistCurve.pdf}&
%		\includegraphics[width=0.24\textwidth]{visuals/MJWangleCurve.pdf}\\
%		Distance Jeans (F) & Normals Jeans (F) & Distance Jeans (M) & Normals Jeans (M) \\
%	\end{tabular}
%	\caption{Average precision curves for vertex distance and face normal angle error for jeans.}
%	\label{fig:precisionJeans}
%\end{figure*}		
	

==> fig/datasetFig1.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure*}[htp!]
	\centering
	\includegraphics[width=0.8\textwidth]{visuals/Picture1_.png}
	\caption{The illustration of a training sample along with a representative prediction result.}
	\label{datasetFig1}
\end{figure*}

==> fig/visRes1.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure*}[h!]
	\centering
	\begin{subfigure}[b]{0.8\textwidth}
		\includegraphics[width=\textwidth]{visuals/visComp/MTNN_monkey_CSR2597A_Pred_front.png}
		\caption{The predictions by \Local~for monkey motion in male t-shirt dataset.}
		\label{fig:visRes1_front_Pred}
	\end{subfigure}
	\begin{subfigure}[b]{0.8\textwidth}
		\includegraphics[width=\textwidth]{visuals/visComp/MTNN_monkey_CSR2597A_GT_front.png}
		\caption{PBS results for monkey motion in male t-shirt dataset.}
		\label{fig:visRes1_front_GT}
	\end{subfigure}
	\begin{subfigure}[b]{0.8\textwidth}
		\includegraphics[width=\textwidth]{visuals/visComp/FTNN_walking_long_csr4237a_Pred_front.png}
		\caption{The predictions by \Local~for walking motion in female t-shirt dataset.}
		\label{fig:visRes1_back_Pred}
	\end{subfigure}
	\begin{subfigure}[b]{0.8\textwidth}
		\includegraphics[width=\textwidth]{visuals/visComp/FTNN_walking_long_csr4237a_GT_front.png}
		\caption{PBS results for walking motion in female t-shirt dataset.}
		\label{fig:visRes1_back_GT}
	\end{subfigure}

	\begin{subfigure}[b]{0.8\textwidth}
		\includegraphics[width=\textwidth]{visuals/visComp/MJNN_monkey_nl_1207a_Pred_back.png}
		\caption{The predictions by \Local~for monkey motion male-jeans dataset.}
		\label{fig:visRes2_front_Pred}
	\end{subfigure}
	\begin{subfigure}[b]{0.8\textwidth}
		\includegraphics[width=\textwidth]{visuals/visComp/MJNN_monkey_nl_1207a_GT_back.png}
		\caption{PBS results for monkey motion in male-jeans dataset.}
		\label{fig:visRes2_front_GT}
	\end{subfigure}
	\begin{subfigure}[b]{0.8\textwidth}
		\includegraphics[width=\textwidth]{visuals/visComp/FJNN_dance_2_CSR0055A_Pred_front.png}
		\caption{The predictions by \Local~for dance motion in female-jeans dataset.}
		\label{fig:visRes2_back_Pred}
	\end{subfigure}
	\begin{subfigure}[b]{0.8\textwidth}
		\includegraphics[width=\textwidth]{visuals/visComp/FJNN_dance_2_CSR0055A_GT_front.png}
		\caption{PBS results for dance motion in female-jeans dataset.}
		\label{fig:visRes2_back_GT}
	\end{subfigure}
	\caption{Visual results for several body poses in different garment-gender combinations.}
	\label{fig:visRes}
\end{figure*}


==> fig/visRes2.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure*}[h!]
	\centering
	\begin{subfigure}[b]{0.8\textwidth}
		\includegraphics[width=\textwidth]{visuals/visComp/MJNN_monkey_CSR2111A_Pred_front.png}
		\caption{The predictions by \Local.}
		\label{fig:visRes1_front_Pred}
	\end{subfigure}
	\begin{subfigure}[b]{0.8\textwidth}
		\includegraphics[width=\textwidth]{visuals/visComp/MJNN_monkey_CSR2111A_GT_front.png}
		\caption{PBS results.}
		\label{fig:visRes1_front_GT}
	\end{subfigure}
	\begin{subfigure}[b]{0.8\textwidth}
		\includegraphics[width=\textwidth]{visuals/visComp/MJNN_monkey_CSR2111A_Pred_back.png}
		\caption{The predictions by \Local.}
		\label{fig:visRes1_back_Pred}
	\end{subfigure}
	\begin{subfigure}[b]{0.8\textwidth}
		\includegraphics[width=\textwidth]{visuals/visComp/MJNN_monkey_CSR2111A_GT_back.png}
		\caption{PBS results.}
		\label{fig:visRes1_back_GT}
	\end{subfigure}
	\caption{Visual results from monkey motion for male jeans.}
	\label{fig:visRes1}
\end{figure*}


==> tex/3_dataset.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\section{Dataset Generation}
\label{sec:dataset}

To train and test the model introduced the previous section, we used the NVidia physically-based simulator NvCloth~\cite{Nvcloth} to fit four 4 different garments---female jeans, male jeans, female t-shirt, and male t-shirt represented  by 3D triangulated meshes with 5351, 5351, 5278, and 5442 vertices, respectively---on bodies from the  CAESAR dataset~\cite{Allen03}. The 80 female and 98 male bodies are represented by 6449-vertex meshes.

Each body in the CAESAR dataset comes in only one pose, genrally the T-pose. To provide a variety of poses for our dataset, we used the CMU mocap database~\cite{CMU} to animate yoga, dance, monkey, and walking motions. We selected 25 poses for each activity and ran the simulator for all 4 garments on each. However, we had to exclude yoga motions for the jeans because the sharp body curvatures resulted in simulation failures.

Since the garment has a fixed size, we must first prune the CAESAR dataset to only keep the bodies that the garment can fit to realistically. We uniformly sample the CEASAR bodies in the interval of 0.8 and 1.4 m of belt circumference, leaving us with 80 female and 98 male bodies in total. Finally, for each combination, we selected 60\% of the results for training purposes, 20\% for validation, and 20\% for testing.
\PF{There should be images in the supplementary material that describe all this.}
